The iWildCam 2021 Competition Dataset

Camera traps enable the automatic collection of large quantities of image data. Ecologists use camera traps to monitor animal populations all over the world. In order to estimate the abundance of a species from camera trap data, ecologists need to know not just which species were seen, but also how many individuals of each species were seen. Object detection techniques can be used to find the number of individuals in each image. However, since camera traps collect images in motion-triggered bursts, simply adding up the number of detections over all frames is likely to lead to an incorrect estimate. Overcoming these obstacles may require incorporating spatio-temporal reasoning or individual re-identification in addition to traditional species detection and classification. We have prepared a challenge where the training data and test data are from different cameras spread across the globe. The set of species seen in each camera overlap, but are not identical. The challenge is to classify species and count individual animals across sequences in the test cameras.

==> authors.tex <==
Sara Beery*$^\dagger$, Arushi Agarwal*, Elijah Cole*$^\dagger$, Vighnesh Birodkar$^\dagger$\\
\begin{tabular}{ccc}
California Institute of Technology* & Google$^\dagger$ 

\end{tabular}
